The Compressed Overlap Index

For analysing text algorithms, for computing superstrings, or for testing random number generators, one needs to compute all overlaps between any pairs of words in a given set. The positions of overlaps of a word onto itself, or of two words, are needed to compute the absence probability of a word in a random text, or the numbers of common words shared by two random texts. In all these contexts, one needs to compute or to query overlaps between pairs of words in a given set. For this sake, we designed COvI, a compressed overlap index that supports multiple queries on overlaps: like computing the correlation of two words, or listing pairs of words whose longest overlap is maximal among all possible pairs. COvI stores overlaps in a hierarchical and non-redundant manner. We propose an implementation that can handle datasets of millions of words and still answer queries efficiently. Comparison with a baseline solution - called FullAC - relying on the Aho-Corasick automaton shows that COvI provides significant advantages. For similar construction times, COvI requires half the memory FullAC, and still solves complex queries much faster.

==> macros.tex <==
\newcommand{\fyle}[1]{{\texttt{#1}}}
\newcommand{\namelabel}[1]{{\textsc{#1}}}
\newcommand{\vmit}[1]{\mbox{\textit{#1}}}


\newcommand{\EHOG}{{\namelabel{EHOG}}}
\newcommand{\HOG}{{\namelabel{HOG}}}
\newcommand{\LOUDS}{{\namelabel{LOUDS}}}
%\newcommand{\COvI}{{\namelabel{COvI}}}
\newcommand{\COvI}{{\formatfonc{COvI}}}
\newcommand{\covi}{{\formatfonc{COvI}}}
\newcommand{\AC}{{\formatfonc{Full AC}}}
\newcommand{\fullac}{{\formatfonc{Full AC}}}
%\newcommand{\AC}{{\namelabel{Full AC}}}
\newcommand{\BP}{{\namelabel{BP}}}

\newcommand{\method}[1]{{\textsf{#1}}}

%\newcommand{\D}{}
\newcommand{\D}{\hphantom{0}}

\newcommand{\etal}{\textit{et al.}}
\newcommand{\ie}{\emph{i.e.}}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\lgr}[1]{\vert #1 \vert}
\newcommand{\gb}[1]{{\mbox{$#1$~GB}}}
\newcommand{\mb}[1]{{\mbox{$#1$~MB}}}
\newcommand{\kb}[1]{{\mbox{$#1$~kB}}}



==> tbl/tbl_data.tex <==
\begin{tabular}{lc cc cc c}
\toprule
\multirow{2}{*}{File Name}		&& \multirow{2}{*}{Size (Megabytes)} 	&& Number 	 && \multirow{2}{*}{$\sigma$}  \\
					&&					&& of Words      &&                           
\\	
\midrule
\fyle{DNA $25$-mers}			&& \D{ }$447.0$		&&	$18{,}028{,}835$	&& \D$16$  
\\
\fyle{DNA $50$-mers}			&& \D{ }$916.6$		&&	$18{,}844{,}684$	&& \D$16$  
\\
%\fyle{DNA $75$-mers}			&& $1{,}374.46$		&&	$18{,}963{,}485$	&& \D$16$  
%\\
\fyle{DNA $100$-mers}			&& $1{,}830.1$		&&	$19{,}000{,}429$	&& \D$16$  
\\
\midrule
\fyle{PROTEINS $25$-mers}		&& \D{ }$371.3$		&&	$14{,}975{,}787$	&& \D$27$  
\\
\fyle{PROTEINS $50$-mers}		&& \D{ }$685.3$		&&	$14{,}090{,}763$	&& \D$27$  
\\		
%\fyle{PROTEINS $75$-mers}		&& \D{ }$943.44$	&&	$13{,}016{,}688$	&& \D$27$  
%\\
\fyle{PROTEINS $100$-mers}		&& $1{,}147.1$		&&	$11{,}908{,}565$	&& \D$27$  
\\
\midrule
\fyle{ENGLISH $25$-mers}		&& \D{ }$438.7$		&&	$17{,}692{,}377$	&& $239$  
\\
\fyle{ENGLISH $50$-mers}		&& \D{ }$868.9$		&&	$17{,}864{,}478$	&& $239$  
%\\
%\fyle{ENGLISH $75$-mers}		&& $1{,}299.28$		&&	$17{,}926{,}269$	&& $239$  
\\
\fyle{ENGLISH $100$-mers}		&& $1{,}729.9$		&&	$17{,}960{,}037$	&& $239$  
\\
\bottomrule
\end{tabular}
			


==> tbl/tbl_nodes.tex <==

\begin{tabular}{lc cc cc c}
\toprule
\multirow{2}{*}{File Name}		&& Nodes of 	&& Nodes of 	 && \% Of the Total \\
					&& the $AC$	&& the {\COvI}   &&                           
\\	
\midrule
\fyle{DNA $25$-mers}			&& \D{ }$248{,}356{,}644$		&&	\D$70{,}357{,}220$	&& $28.3$ 
\\
\fyle{DNA $50$-mers}			&& \D{ }$713{,}491{,}283$		&&	$159{,}625{,}885$	&& $22.4$
\\
\fyle{DNA $100$-mers}			&& $1{,}661{,}261{,}512$		&&	$335{,}429{,}455$	&& $20.2$
\\
\midrule
\fyle{PROTEINS $25$-mers}		&& \D{ }$304{,}470{,}523$ 		&&	\D$89{,}581{,}658$	&& $29.4$
\\
\fyle{PROTEINS $50$-mers}		&& \D{ }$628{,}268{,}391$		&&	$161{,}891{,}030$	&& $25.8$
\\		
\fyle{PROTEINS $100$-mers}		&& $1{,}111{,}355{,}314$		&&	$242{,}678{,}948$	&& $21.8$
\\
\midrule
\fyle{ENGLISH $25$-mers}		&& \D{ }$288{,}569{,}455$		&&	\D$92{,}402{,}990$	&& $32.0$
\\
\fyle{ENGLISH $50$-mers}		&& \D{ }$734{,}042{,}063$		&&	$200{,}620{,}965$	&& $27.3$
\\
\fyle{ENGLISH $100$-mers}		&& $1{,}630{,}202{,}927$		&&	$415{,}286{,}652$	&& $25.5$
\\
\bottomrule
\end{tabular}

==> tbl/tbl_ov_1.tex <==

\begin{tabular}{l  ccc  ccc  ccc}
\toprule
File Name		& \multicolumn{3}{c}{\fyle{DNA}} & \multicolumn{3}{c}{\fyle{PROTEINS}} & \multicolumn{3}{c}{\fyle{ENGLISH}}
\\
\vmit{k-mer} value 	& $25$ & $50$ & $100$ & $25$ & $50$ & $100$ & $25$ & $50$ & $100$
\\
\midrule 
$\vmit{overlap}(x,y)$		& \multirow{2}{*}{\D$3.42$} & \multirow{2}{*}{\D$5.22$} & \multirow{2}{*}{\D$9.38$}   
				& \multirow{2}{*}{\D$3.12$} & \multirow{2}{*}{\D$6.54$} & \multirow{2}{*}{$11.17$}    
				& \multirow{2}{*}{\D$3.80$} & \multirow{2}{*}{\D$6.61$} & \multirow{2}{*}{$11.88$}	
\\ 
(microseconds)	
\\ 		
\\
$\vmit{all-overlap}(x,y)$	& \multirow{2}{*}{\D$3.40$} & \multirow{2}{*}{\D$5.27$} & \multirow{2}{*}{\D$9.37$}   
				& \multirow{2}{*}{\D$3.14$} & \multirow{2}{*}{\D$6.54$} & \multirow{2}{*}{$11.12$}    
				& \multirow{2}{*}{\D$3.78$} & \multirow{2}{*}{\D$6.60$} & \multirow{2}{*}{$11.89$}		
\\
(microseconds)	
\\
\midrule
$\vmit{all-right-overlaps}(x)$ 	& \multirow{2}{*}{$17.53$} & \multirow{2}{*}{$27.45$} & \multirow{2}{*}{$45.31$}   
				& \multirow{2}{*}{$12.81$} & \multirow{2}{*}{$19.78$} & \multirow{2}{*}{$27.13$}    
				& \multirow{2}{*}{$19.82$} & \multirow{2}{*}{$32.49$} & \multirow{2}{*}{$55.00$}	
\\ 
(seconds)	
\\ 		
\\ 
$\vmit{all-left-overlaps}(x)$, 	& \multirow{2}{*}{$14.62$} & \multirow{2}{*}{$28.15$} & \multirow{2}{*}{$52.66$}   
				& \multirow{2}{*}{$12.42$} & \multirow{2}{*}{$21.74$} & \multirow{2}{*}{$32.07$}    
				& \multirow{2}{*}{$19.95$} & \multirow{2}{*}{$34.84$} & \multirow{2}{*}{$64.21$}	
\\ 
(seconds)	
\\ 		
\midrule
$\vmit{max-overlap()}$		& \multirow{2}{*}{\D$2.55$} & \multirow{2}{*}{\D$2.84$} & \multirow{2}{*}{\D$3.00$}   
				& \multirow{2}{*}{\D$2.28$} & \multirow{2}{*}{\D$2.34$} & \multirow{2}{*}{\D$2.14$}    
				& \multirow{2}{*}{\D$2.70$} & \multirow{2}{*}{\D$2.98$} & \multirow{2}{*}{\D\D$3.23$}	
\\
(seconds)	
\\
\bottomrule
\end{tabular}

==> tbl/tbl_times.tex <==
%\scriptsize
\begin{tabular}{>{\columncolor[gray]{.6}}l  ccc  ccc  ccc}
  \rowcolor[gray]{.6}
  File Name		& \multicolumn{3}{c}{\fyle{DNA}} & \multicolumn{3}{c}{\fyle{PROTEINS}} & \multicolumn{3}{c}{\fyle{ENGLISH}}
  \\
  \rowcolor[gray]{.6}
  \vmit{k-mer} value 	& $25$ & $50$ & $100$ & $25$ & $50$ & $100$ & $25$ & $50$ & $100$
  \\
  Build \vmit{trie} $T$ & \multirow{2}{*}{$15.1$} & \multirow{2}{*}{$36.2$} & \multirow{2}{*}{{ }$74.4$}   
			& \multirow{2}{*}{\D$18.0$} & \multirow{2}{*}{\D$37.2$} & \multirow{2}{*}{\D{ }\D$64.8$}    
                        & \multirow{2}{*}{\D$39.1$} & \multirow{2}{*}{\D$66.5$} & \multirow{2}{*}{\D{ }$129.6$}	
  \\ 
  Failure Links $F$	& $112.4$ & $225.5$ & \D{ }$484.2$   
			& $208.6$ & $285.3$ & \D{ }$408.3$ 
                        & $359.9$ & $493.7$ & \D{ }$756.4$
  \\ \& Mark nodes $M$ \\
  Build {\COvI} 	& \D$20.1$ & \D$45.2$ & \D{ }$114.3$   
			& \D$26.3$ & \D$49.3$ & \D{ }\D$87.7$   
                        & \D$38.7$ & \D$76.1$ & \D{ }$145.6$
  \\ 
  \rowcolor[gray]{.8}
  Total time in s.	& \multirow{2}{*}{$147.6$} & \multirow{2}{*}{$306.9$} & \multirow{2}{*}{\D{ }$672.9$}   
			& \multirow{2}{*}{$252.9$} & \multirow{2}{*}{$371.8$} & \multirow{2}{*}{\D{ }$560.8$}   
                        & \multirow{2}{*}{$437.7$} & \multirow{2}{*}{$636.3$} & \multirow{2}{*}{$1{,}031.6$}
  \\
  \rowcolor[gray]{.8}
  {\COvI} space in Mb	& \multirow{2}{*}{$357.7$} & \multirow{2}{*}{$797.2$} & \multirow{2}{*}{$1{,}686.3$}  
			& \multirow{2}{*}{$439.5$} & \multirow{2}{*}{$791.2$} & \multirow{2}{*}{$1{,}212.0$}       
                        & \multirow{2}{*}{$460.8$} & \multirow{2}{*}{$981.8$} & \multirow{2}{*}{$2{,}067.9$}
\end{tabular}


\begin{comment}
  \begin{tabular}{l | cccc | cccc | cccc}
    \toprule
    File Name		& \multicolumn{4}{c}{\fyle{DNA}} & \multicolumn{4}{c}{\fyle{PROTEINS}} & \multicolumn{4}{c}{\fyle{ENGLISH}}
    \\
    \vmit{k-mer} value 	& 25 & 50 & 75 & 100 & 25 & 50 & 75 & 100 & 25 & 50 & 75 & 100
    \\
    \midrule
    Generate the \vmit{trie} (sec)	& \D$15.13$	& \D$36.23$ & 55 & 72 &18&35&48&64    &38&64&88&109	
    \\ &&&&&&&&&&\\
    Compute Failure Links		& \multirow{2}{*}{$112.40$} & \multirow{2}{*}{$225.48$} & 346 & 484 &207&284&348&408 &359&493&627&761
    \\
    and Mark Nodes (sec)
    \\ &&&&&&&&&&\\
    Create {\COvI} (sec)		& \D$20.06$ & \D$45.17$ & 78 & 112 &25&49&70&85   &37&75&116&155
    \\ &&&&&&&&&&\\ 
    \midrule 
    Total Time (seconds)		& $147.59$ & $306.88$ & 482.96 & 672.89 &252.89&371.76&469.42&560.77 &437.68&636.29&835.98&1031.62
    \\
    \midrule
    Space (Megabytes) 		& $357.69$ & $797.22$ & 1260.44 & 1686.28 &439.47&791.18&1039.90&1212.01 &460.80&981.84&1550.51&2067.85
    \\
    \bottomrule
  \end{tabular}
\end{comment}

